Verify with Caution: The Pitfalls of Relying on Imperfect Factuality Metrics

Improvements in large language models have led to increasing optimism that they can serve as reliable evaluators of natural language generation outputs. In this paper, we challenge this optimism by thoroughly re-evaluating five state-of-the-art factuality metrics on a collection of 11 datasets for summarization, retrieval-augmented generation, and question answering. We find that these evaluators are inconsistent with each other and often misestimate system-level performance, both of which can lead to a variety of pitfalls. We further show that these metrics exhibit biases against highly paraphrased outputs and outputs that draw upon faraway parts of the source documents. We urge users of these factuality metrics to proceed with caution and manually validate the reliability of these metrics in their domain of interest before proceeding.

==> scratch.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
% OLD ADJUSTMENT TABLE %
%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{tabular}{llcccc}
% \toprule
% QE & Source & No Adj. & Quantification Adj. & Quantification tuned & BAcc tuned \\
% \midrule
% average & CNN/DM & 3.9 (3.5) & \cellcolor{green2}15.3 (1.8) & \cellcolor{green3}1.9 (1.5) & \cellcolor{green2}14.8 (3.1) \\
%       & MARCO & 14.4 (12.7) & \cellcolor{green3}7.2 (3.3) & \cellcolor{green3}3.4 (1.4) &                      20.2 (6.8) \\
%       & Recent News & 3.0 (2.4) & 10.5 (3.2) & \cellcolor{green3}2.3 (1.6) & \cellcolor{green2}10.2 (1.9) \\
%       & Yelp & 15.4 (12.2) & \cellcolor{green2}26.9 (8.3) & \cellcolor{green3}6.0 (4.0) & \cellcolor{green2}19.3 (4.5) \\
% \midrule
% worst & CNN/DM & 6.1 (6.1) & \cellcolor{green2}21.5 (3.2) & \cellcolor{green3}4.0 (3.5) & \cellcolor{green2}19.6 (5.7) \\
%       & MARCO & 22.3 (20.6) & \cellcolor{green3}12.1 (6.4) & \cellcolor{green3}6.7 (4.7) & \cellcolor{green2}27.9 (12.4) \\
%       & Recent News & 5.9 (5.6) & 18.8 (7.7) & \cellcolor{green3}5.0 (3.4) & \cellcolor{green2}18.8 (4.2) \\
%       & Yelp & 29.7 (22.2) & \cellcolor{green2}43.7 (21.7) & \cellcolor{green3}13.1 (6.7) & \cellcolor{green2}31.2 (11.3) \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Comparison of adjustment methods on RAGTruth:} Numbers denote the average cross-validated quantification error. For cross-validation, we use out one system to set the error rates for adjustment with quantification / tune the threshold. The adjustment/tuning is used to quantify the error rates of the remaining 5 held-out systems. The numbers in parantheses denote the best (minimum) quantification error achievable by adjustment/tuning. Threshold tuning to minize quantification error reduces both the average and worst quantification error consistently. Tuning for balanced accuracy may reduce quantification error in one fold but not with cross-validation.}


%%%%%%%%%%%%%%%%%%%%%%%%
%  CHUNKING DIFF TABLE %
%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[]
% \centering
% \small
% \begin{tabular}{lrrrr}
% \toprule
% {} & \multicolumn{2}{l}{0 --> 1} & \multicolumn{2}{l}{1 --> 0} \\
% {} & ROUGE\_diff = 0 & ROUGE\_diff > 0 & ROUGE\_diff = 0 & ROUGE\_diff > 0 \\
% dataset         &                &                &                &                \\
% \midrule
% AggreFact-CNN   &            1.2 &            0.0 &            0.6 &           23.1 \\
% AggreFact-XSum  &            1.0 &            0.0 &            3.0 &            9.6 \\
% TofuEval-MediaS &            2.1 &            1.4 &            5.6 &           14.4 \\
% TofuEval-MeetB  &            2.7 &            3.4 &            5.4 &           18.3 \\
% Wice            &            1.9 &            1.1 &            8.9 &           13.2 \\
% ClaimVerify     &            1.4 &            5.2 &            2.6 &            4.7 \\
% ExpertQA        &            1.3 &            2.5 &            1.9 &           11.9 \\
% Lfqa            &            1.1 &            2.3 &            1.6 &            8.0 \\
% RAGTruth-CNN/DM &            0.8 &            1.0 &            3.1 &           14.7 \\
% RAGTruth-News   &            0.7 &            0.0 &            2.2 &           21.5 \\
% RAGTruth-Yelp   &            1.5 &            2.3 &            8.0 &           20.3 \\
% \bottomrule
% \end{tabular}
% \caption{Percentage of changes in predictions when chunking causes a change in $\text{ROUGE}_\text{diff}$}
% \label{tab:rouge_diff_pred_change}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%
% OLD ROUGE GRAPHS %
%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.4\textwidth]{latex/images/llmaggrefact-calibration-vs-rouge-p-quantile-summ-main.png}
%     \caption{\textbf{ROUGE-2 precision vs prediction behavior of AutoAIS metrics on summarization tasks:} ROUGE-2-precision is (anti-)correlated with true (negative)positive rate, i.e. metrics mislabel attributable generations with low ROUGE and unattributable generations with high ROUGE-2 precision. Metrics without chunking seem well-calibrated on the summarization tasks; the metric under-predicts the label 1 (attributable) when documents are chunked.
%     }
%     \label{fig:rouge-calibration-summ}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.4\textwidth]{latex/images/llmaggrefact-calibration-vs-rouge-p-quantile-non-summ-main.png}
%     \caption{\textbf{ROUGE-2 precision vs prediction behavior of AutoAIS metrics on non-summarization tasks:} ROUGE-2-precision is (anti-)correlated with true (negative)positive rate, i.e. metrics mislabel attributable generations with low ROUGE and unattributable generations with high ROUGE-2 precision. \gptf has good calibration, and both \bespoke variants have poor calibration on the non-summarization tasks.
%     }
%     \label{fig:rouge-calibration-non-summ}
% \end{figure}

% Next, the metrics that can handle long documents (\bespoke and \gptf) have well-calibrated predictions in different quantiles of ROUGE-2 precision; their rate of predicting the label "attributable" matches the ground-truth rate in the different bins. However, \bespoke with chunking under-predicts the positive (attributable) class; we will look into this behavior in the next section.

%%%%%%%%%%%%%%%%
% TABLE FORMAT %
%%%%%%%%%%%%%%%%
\begin{table*}
\centering
\tiny
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc|ccc|}
\toprule
GT Order & \multicolumn{3}{c|}{GPT-4-turbo} & \multicolumn{3}{c|}{GPT-3.5-turbo} & \multicolumn{3}{c|}{Bespoke-7B} & \multicolumn{3}{c|}{Bespoke-7B (cs=500)} & \multicolumn{3}{c|}{MiniCheck-FT5} & \multicolumn{3}{c|}{MiniCheck-Roberta} & \multicolumn{3}{c|}{AlignScore} \\
 & > & = & < & > & = & < & > & = & < & > & = & < & > & = & < & > & = & < & > & = & < \\
\midrule
\midrule
\%Err & \multicolumn{3}{c|}{20.0} & \multicolumn{3}{c|}{40.0} & \multicolumn{3}{c|}{33.3} & \multicolumn{3}{c|}{33.3} & \multicolumn{3}{c|}{33.3} & \multicolumn{3}{c|}{26.7} & \multicolumn{3}{c|}{26.7} \\
\%Maj. Err & \multicolumn{3}{c|}{0.0} & \multicolumn{3}{c|}{0.0} & \multicolumn{3}{c|}{0.0} & \multicolumn{3}{c|}{0.0} & \multicolumn{3}{c|}{0.0} & \multicolumn{3}{c|}{0.0} & \multicolumn{3}{c|}{0.0} \\
\bottomrule
\end{tabular}
\caption{\textbf{TofuEval-MeetingBank: Inconsistency in system-pair ranking based on claim-level error rates for systems.} We report a confusion matrix of pairwise system ranking decisions. We measure inconsistencies between the ranking based on the labeled error rate and the ranking based on the predicted error rate. For a system pair (s1, s2),  `=' indicates no significant difference between s1 and s2, `<' indicates s1 has a lower error rate than s2, and `>' indicates s1 has a higher error rate than s2. When a metric predicts a significant but opposite ranking between a pair, we count it as a
Major Error. Significance is computed with the two-proportion z-test and p\_value < 0.05.}
\label{tab:meetb-instance-ranking-error}
\end{table*}
